Wireless Sensor Networking for Rain-fed Farming Decision Support

Wireless sensor networks (WSNs) can be a valuable decision-support tool for farmers. This motivated our deployment of a WSN system to support rain-fed agriculture in India. We defined promising use cases and resolved technical challenges throughout a two-year deployment of our COMMON-Sense Net system, which provided farmers with environment data. However, the direct use of this technology in the field did not foster the expected participation of the population. This made it difficult to develop the intended decision-support system. Based on this experience, we take the following position in this paper: currently, the deployment of WSN technology in developing regions is more likely to be effective if it targets scientists and technical personnel as users, rather than the farmers themselves. We base this claim on the lessons learned from the COMMON-Sense system deployment and the results of an extensive user experiment with agriculture scientists, which we describe in this paper.

==> analysis.tex <==
\section{Experiment Results} \label{sectionresults}

\subsection{Questionnaires}
An extensive list of the data and their interpretation can be found in
\cite{PanchardRS08}. All participants but one identified environmental
information as an important input for the study of rain-fed farming. As for
parameters, soil water content and temperature are considered the most
important to monitor, as shown in Fig. \ref{DetailedParameter}.

\begin{figure}[!ht]
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=2.5in]{../../images/detailedParameter.pdf}\\
  \caption{Critical parameters as identified by the experiment's participants}\label{DetailedParameter}
\end{figure}

The participants also had to characterize the parameters they chose with regard
to the required spatial density, sampling frequency, and tolerated error.
Regarding spatial density,  the parameters can be classified into two
categories: the parameters considered with a low spatial variability, i.e. one
kilometer and above, such as temperature, rain fall and atmospheric pressure.
And the parameters demanding high spatial variability (from 500m down to one
hectare): only soil moisture belongs to this category. Interestingly, soil type
shows a bimodal result, about half the users considering that a single
measurement point is enough, and the other half considering that it should be
performed at least every few hundred meters.

The required measurement frequency shows a wider distribution. It is
interesting to note, however, that in all cases but one (soil moisture), the
lower limit is the day. Only for soil moisture were hourly or more frequent
measurements deemed appropriate, and only for a minority of users (less than 10
percent).

As for the error tolerance for each parameter, the participants tend to require
high precision (less than five percent error).

%The results relative to the important parameters are consistent with those of
%the general questionnaire. The only notable difference is that temperature is
%now considered more important than soil moisture, which still remains the
%second most important parameter, however. It is interesting to note that
%temperature is not considered a constraint in itself, but is recognized as an
%important parameter to monitor other constraints.

\begin{figure}[!ht]
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=3.0in]{../../images/detailedConstraintPerCrop.pdf}\\
  \caption{Detailed Questionnaire:  Constraints per crop type (expressed in number of answers)}\label{DetailedPerCrop}
\end{figure}

Fig. \ref{DetailedPerCrop} shows the parameter distribution per crop. This
table confirms that for each crop the parameters to take into account are the
same, except pest, which is not considered to be an issue for ragi.

The results about parameters, their variability and error tolerance are
consistent between the general questionnaire and the detailed questionnaire. In
other terms, users did not noticeably change their mind after using the web
application. The next section clearly explains why.

\subsection{User Activity Logging} \label{quantitative}
This is the set of metadata that was generated by the logging of participants'
interactions with the web application. This part of the experiment led to
inconclusive results. Out of the 30 participants, only six actually used the
on-line application at some point. All of them were PhD students and post-docs.
No senior researcher spontaneously used the on-line application.

The participants who used the application did an average of 3 queries to the
system, mostly to look at the soil moisture status.

This paradoxical disinterest for the on-line application is discussed in the
next question. It made the debriefing meetings very important, in order to
understand the mismatch between the interest manifested in the survey and the
actual use of the application.

\subsection{Debriefing Meetings}
Initially, the debriefing meetings were intended to gather the opinions of the
participants in a more informal manner than during the experiment. However, in
light of the mismatch mentioned in the previous section, they became a crucial
element of the experiment. The goal was to find out why the users had not used
the application as expected, and to assess their real level of interest.

%The meetings were conducted with 8 Professors (out of the 10 who initially
%answered the survey). Additionally, we discussed the application with a top NGO
%executive, and a local official of the agriculture department of Karnataka.

Instead of asking these questions directly, which would have been likely to
bias the answers, we chose to address concrete use cases. If people were able
to come up with original use cases, that meant they had conducted a reflection
about the tool. Moreover, we could then talk concretely about upcoming
partnerships, an extra- measure of their interest, and a critical conditions
for the continuation of the project.

The results were encouraging. We found four compelling use cases, and in each
case a concrete interest in using the technology provided. Precise details
about the requirements of each use case can be found in \cite{PanchardRS08}.

\subsubsection{Soil Science}
Provided we can adapt nutrient sensors to the wireless nodes, there is research
to be conducted in the response at the root zone to different strategies of
nutrient application and irrigation. The main objective would be to observe the
variation in nitrogen , phosphorus and potassium content, in the context of
nutrient dynamics under a system of multiple crops and trees.

%Appropriate sensors are of interest in order to understand the dynamics of
%nutrients and soil moisture, soil PH, etc. Experiment would be meaningful if
%conducted in the following way:
%\begin{itemize}
%  \item 4 ha divided in 4 plots, 10 sensors per plot.
%  \item Sensors placed at 2 different depths
%  \item Experiment should last 2-3 years minimum
%  \item Bi-weekly measurements \footnote{For research purposes, having multiple measures per day would be useful, but
%that would not give meaningful results from an agriculture point-of-view,
%because the time-scale of farming operations is much larger.}
%\end{itemize}
%
%The interviewee is willing to undertake such an experiment, and encouraged us
%to contact him when we have identified the proper sensors for nutrient
%concentration (\textbf{do these exist?}).

\subsubsection{Entomology}

The observation of pests present in the crop field shows that their activity
depends on the weather, especially rain fall, soil moisture and soil
temperature. There is a clear correlation between the rain patterns and the
emergence of adults of the insects from the soil. %This happens in a fixed time
%of the year between the last week of April and the end of June. If there is
%rain before April 20th, then there is no emergence. Moreover, after October all
%the larvae enter pupation and emerge as adults after 20 days. If the soil
%moisture conditions are not favorable to them until the end of June, a large
%percentage of the population might die.
%
%Another pest, the Red Hairy Caterpillar has a similar biology but 2 months later
%than the white grubs. Emergence happens in two cycles, one in early July and
%the second in late September.

The hypothesis to verify is whether the insect's activity depends on soil
moisture evolution and accumulation of soil heat in the weeks prior to
emergence. If the soil moisture conditions are not favorable to them during
pupation, a large percentage of the population might die.

Soil moisture, temperature sensors in specific regions of endemic populations
of these pests (sampling various soil texture typologies) will help to
investigate, understand their biology . This would make it possible to provide
advance information on the intensity of pest damage to farmers.

%The interviewee expressed keen interest on the usage of WSNs, in a first stage
%to test the technology's reliability and effectiveness.

\subsubsection{Crop Physiology}
This use case is about the precise assessment of the ratio between the water
that is transpired by the plant and the water that is evaporated, in other
terms the plant's water efficiency. The possibility to achieve crop improvement
through selection would have a positive impact on yields achieved in rain-fed
farming. For this, it is necessary to test plants with different genotypes
obtained by cross-breeding and to assess which one has the best ratio of
biomass production per water used.

The method used for this test today is gravimetric method. For this, plants in
pots are used.  The pots are filled daily with water up to field capacity. The
next day, they are weighted to assess the water lost in evapo-transpiration.
Bare plots are used as a benchmark to assess the effect of pure evaporation.

The goal is to replace the gravimetric method with soil moisture sensors that
would give directly the volumetric content of water of the soil. The tedious
weighting procedure could then be avoided.

%A typical experience contains 120-200 pots. Each pot should contain 1-4 probes
%(ECH2O) connected to one wireless sensor. The experiment duration is typically
%80 days from plant sowing (out of which 50 days of measures) The number of
%measures should be at least 4 per day, without upper limit.
%
%His expressed interest is high. The interviewee would like to conduct as soon
%as possible a first experiment with 30 pots, as a proof of concept.



\subsubsection{Water management}
For a large NGO conducting applied research in the area of rain-fed farming,
wireless sensor networks are perceived as a promising validation tool. Two
experiments are envisioned:

\begin{enumerate}
  \item the possibility to increase soil water-retention capacity through different
measures, such as fertilizer, mulching, etc.
  \item assessing the efficiency of underground drip irrigation. Here, the goal is
to bring the water directly to the root zone of the plant.
\end{enumerate}

For both experiments, soil moisture is the ultimate measure of success or
failure.

%A second use case distinct from research validation is information sharing in
%rural kiosks. The NGO implemented a network of internet kiosks in several
%districts of Karnataka. At the central server, extension specialists are
%analyzing data they receive from local kiosks in the villages. This data
%consists in questions and environmental information. Then, they redistribute
%the information they analyzed to the kiosks. Obtaining live data about soil
%moisture content for different types of soil would be an interesting
%complementary source.

%The BAIF executive with whom we spoke expressed keen interest. In a first
%phase, BAIF is interested in 100 sensors minimum.


%\subsubsection{Meetings that did not lead to a use case}
%Prof. Bhaskar, from the forestry department, expressed no interest in the
%application. He mentioned having published long ago a paper that reported on an
%experiment of monitoring soil moisture levels in a crop and tree interaction.
%For measurements they used neutron probes. He understands the utility of
%sensors, but sees no interest in spatial and time diversity.
%
%A Professor in the micro-biology department redirected us to a junior
%collaborator, who exposed two research activities where environmental
%information can be useful:
%
%\begin{itemize}
%  \item Effect of microbial activity on soil nutrition. Environmental parameters have
%an effect on the evolution of nutrients in the soil
%  \item Disease-causing organisms: Observe the conditions in which these organisms
%(typically aerial micro-flora) develop. Environmental parameters may condition
%the outbreak of an epidemic
%\end{itemize}
%
%Typically, research in this area is done in micro-plots. The granularity is
%one-reading per week The parameters of primary interest are soil and air
%temperature, soil moisture and humidity. When prompted, the interviewee
%mentioned other parameters of possible interest, such as wind
%direction/intensity, sun radiance and precipitation.
%
%The interviewee never seemed to think sensor networks could be useful in this
%context. When prompted, she acknowledged that the size of the experiments was
%constrained by the difficulty to obtain parameters at a satisfying rate, but
%did not really consider the use of WSNs in this framework.
%
%Prof. Bhaskar (Crop Physiology, UAS) recognized environmental information as
%useful for post-mortem analysis in case of crop failure - assess crop
%suitability - evaluate date of planting. The type of data needed is soil
%moisture (several stations), plus one weather station. A typical type of
%deployment is nodes scattered in a circular pattern, with typically 200m
%between the stations. The number of sensors depends on soil type and soil
%variability. The depth of the sensor placement for particular plants depends on
%the type of crop.
%
%However, no precise use case emerged during this meeting. Prof. Bhaskar was not
%convinced that the time variability of the environmental parameters would
%justify the deployment of a wireless sensor network.
%
%Prof. Narayana Gowda is conducting applied studies on the productivity increase
%through appropriate agricultural management techniques. His work spans 72
%villages in the Bangalore greater area. The project uses one automatic weather
%station. Before using sensors, he wants to understand a profitable use case of
%information using sensors.
%
%Dr. R. Reddy, joint-director of the agriculture department of Karnataka state,
%kindly participated to our survey. However, his position was clear. Conducting
%applied research is beyond the mandate of a governmental  agency, which is only
%concerned by extension, i.e. information relaying from the scientific community
%to the farmers. Consequently, we did not ask him to fill the on-line
%questionnaires.


==> bibliography.tex <==
%%**************************************************************
%%\bibliographystyle{unsrt}
%\bibliographystyle{IEEEtran}
%%\bibliography{//icsil1-files/LCA/Users/jpanchar/Work/COMMON-Sense/COMMONSense}%without the .bib
%\bibliography{../../../../COMMONSense}%without the .bib
%%**************************************************************

\begin{thebibliography}{10}
\providecommand{\url}[1]{#1} \csname url@rmstyle\endcsname
\providecommand{\newblock}{\relax} \providecommand{\bibinfo}[2]{#2}
\providecommand\BIBentrySTDinterwordspacing{\spaceskip=0pt\relax}
\providecommand\BIBentryALTinterwordstretchfactor{4}
\providecommand\BIBentryALTinterwordspacing{\spaceskip=\fontdimen2\font plus
\BIBentryALTinterwordstretchfactor\fontdimen3\font minus
  \fontdimen4\font\relax}
\providecommand\BIBforeignlanguage[2]{{%
\expandafter\ifx\csname l@#1\endcsname\relax
\typeout{** WARNING: IEEEtran.bst: No hyphenation pattern has been}%
\typeout{** loaded for the language `#1'. Using the pattern for}%
\typeout{** the default language instead.}%
\else \language=\csname l@#1\endcsname \fi #2}}

\bibitem{DiwikaraC07}
H.~Diwikara and M.~Chandrakanth, ``{Beating negative externality through
  groundwater recharge in India: a resource economic analysis},''
  \emph{Environment and Development Economics, Cambridge University Press},
  vol.~12, pp. 271--296, 2007.

\bibitem{GadgilAR99}
S.~Gadgil, Y.~P. Abrol, and P.~Rao, ``{On growth and Fluctuation of Indian
  Foodgrain Production},'' \emph{Current Science}, 1999.

\bibitem{Abrol96}
I.~Abrol, ``{India's agriculture scenario},'' \emph{Climate variability and
  agriculture}, pp. 19--25, 1996.

\bibitem{Mishra06}
\BIBentryALTinterwordspacing S.~Mishra, ``{Suicide of Farmers in
Maharashtra},'' \emph{Indira Gandhi
  Institute of Development Research}, 2006. [Online]. Available:
  \url{citeseer.nj.nec.com/557578.html}
\BIBentrySTDinterwordspacing

\bibitem{RaoGRG04}
S.~Rao, M.~Gadgil, R.~Krishnapura, A.~Krishna, M.~Gangadhar, and S.~Gadgil,
  ``{Information Needs for Farming and Livestock Management in Semi-arid Tracts
  of Southern India},'' {CAOS, IISc}, Tech. Rep. AS 2, September 2004.

\bibitem{WarkCSKGCVSB07}
T.~Wark, P.~Corke, P.~Sikka, L.~Klingbeil, Y.~Guo, C.~Crossman, P.~Valencia,
  D.~Swain, and G.~Bishop-Hurley, ``Transforming agriculture through pervasive
  wireless sensor networks,'' \emph{IEEE Pervasive Computing}, vol.~6, no.~2,
  pp. 50--57, 2007.

\bibitem{PanchardRPHJ07}
J.~Panchard, S.~Rao, T.~V. Prabhakar, J.-P. Hubaux, and H.~S. Jamadagni,
  ``Common-sense net: A wireless sensor network for resource-poor agriculture
  in the semiarid areas of developing countries,'' \emph{Information
  Technologies and International Development}, vol.~4, no.~1, pp. 51--67, 2007.

\bibitem{Heeks02}
R.~Heeks, ``{Information Systems and Developing Countries: Failure, Success and
  Local Improvisations},'' \emph{The Information Society}, 2001.

\bibitem{ECH2O}
``{ECH2O Soil Moisture and Microclimate Monitoring},'' documentation available
  at http://www.ech2o.com/.

\bibitem{BurriRW07}
N.~Burri, P.~von Rickenbach, and R.~Wattenhofer, ``Dozer: ultra-low power data
  gathering in sensor networks.'' in \emph{IPSN}, T.~F. Abdelzaher, L.~J.
  Guibas, and M.~Welsh, Eds.\hskip 1em plus 0.5em minus 0.4em\relax ACM, 2007,
  pp. 450--459.

\bibitem{tinynode}
``{tinynode wireless sensor from Shockfish},'' http://www.tinynode.com.

\bibitem{PanchardRS08}
J.~Panchard, S.~Rao, and S.~Sheshshayee, ``Wireless sensor networks for applied
  research on rain-fed farming in {I}ndia: an exploratory user experiment,''
  Tech. Rep., 2008, available at: http://people.epfl.ch/jacques.panchard.

\bibitem{KimHSM07}
H.~Kim, J.~Hummel, K.~Sudduthb, and P.~Motavalli, ``{Simultaneous Analysis of
  Soil Macronutrients Using Ion-Selective Electrodes},'' Ph.D. dissertation,
  2007.

\bibitem{Panchard06}
J.~Panchard, ``{Computer-assisted Cognition: Using Wireless Sensor Networks to
  Assist the Monitoring of Agricultural Fields},'' {EPFL, Lausanne}, Tech.
  Rep., 2006, available at http://people.epfl.ch/jacques.panchard.

\end{thebibliography}


==> conclusion.tex <==
\section{Conclusion and Future Work}
We performed an experiment about the usefulness and usability of wireless
sensor networks for rain-fed agriculture. The usefulness to provide
finer-grained environmental data for applied research in this field was clearly
identified. The technology gap remains, however, and can only be bridged with a
highly dynamic process of interaction with potential users. Building
appropriate partnerships and exploring the outcomes of medium and long-term
deployments of WSNs is the next step. The interest from the non-governmental
sector is the most promising because it presents the most direct contact with
the intended beneficiaries of this technology: the small land-holding farmers.


==> context.tex <==
\section{The COMMON-Sense Net System} \label{sectioncsn}

\subsection{Challenges and Opportunities}

%% shift down... not clear if COMMONsense net address those
%% concerns - if so, do point it out
%
%However, such an instrumentation has always been costly and
%cumbersome, due to the heavy (often wired) infrastructure, and to the
%intensive human labor necessary to operate and maintain the sensors.
%Wireless sensor networks, which provide both time and space
%variability at an affordable price, allow for these limitations to be
%overcome.

In order to assess the potential of environment monitoring for
rain-fed agriculture and to draw technical constraints from the
appropriate context, we decided to focus on the concern expressed for
crop yield prediction. Semi-structured interviews with agronomists
led to the following \emph{use cases} \cite{PanchardRPHJ07}:

\begin{enumerate}
  \item Deficit irrigation management: based on the water content of the soil,
  it is possible to design irrigation schemes that make use of limited water resources
  \item Assessment of water conservation measures: using residual soil moisture, it is possible assess efficiency of
  measures such as building bunds, planting trees, mulching etc.
  \item Existing crop models validation: using actual values of soil moisture,
  it is possible to evaluate crop models by comparing with predicted values
\end{enumerate}

We opted for all these use cases to be developed in a
\emph{participatory manner} with the local farmers, in order to avoid
the common pitfalls associated with the deployment of information
systems in developing regions \cite{Heeks02}.

\subsection{System Architecture}

The architecture of our WSN system is depicted in
Fig.~\ref{figarchitecture}. So far, we have deployed two clusters for
more than one year (two full cropping seasons) in a farming
environment in the village of Chennakeshavapura (Karnataka)
\cite{PanchardRPHJ07}. They measure and provide a detailed picture of
the soil moisture conditions in 10 homogenous patches, all rain-fed,
with different crop varieties and different soil characteristics. In
addition, one node records air temperature, humidity and atmospheric
pressure over the same period. We detail and justify hereunder the
system's main design characteristics:

\textbf{Reduced and Targeted Data Types:} The main focus being the water
available in the soil for the crop, we designed a simplified data acquisition
board allowing the instrumentation of two soil moisture probes of the ECH2O
\cite{ECH2O} type, so that the top and bottom of the plant's root zone could be
monitored.

\textbf{Power Management:} We considered the use of solar panels but ruled it
out because of the exposure of such hardware to theft and tampering. Whereas a
wireless sensor in a box can be camouflaged in an outdoor field, a solar panel
has to stand prominently and is easily identified as an object of value. We
turned instead to an original MAC plus routing scheme, Dozer \cite{BurriRW07}.
Our most recent tests indicate a lifetime of more than 7 months (more than one
cropping season) for nodes deployed with this cross-layer protocol in the
conditions of our experiment.

\textbf{Periodical Data Collection:} Because we were interested in the
continuous evolution of phenomena (in particular, water content in the soil),
we chose a periodic data collection model that allowed for the logging of
extended data sets in a centralized database for later retrieval and analysis.
Because of the uncertainty regarding the necessary time resolution, the data
sampling period was set to two minutes. This value is higher than needed a
priori by any agricultural application, but as it was compatible with the
expected life-time of the network, it was chosen as a benchmark from which to
assess the ideal data rate a posteriori.


\begin{figure}
\centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=3.0in]{csn_new.jpg}\\
  \caption{COMMONSense Net system architecture}\label{figarchitecture}
\end{figure}

\textbf{Sparse Network:} 2-3 sensors were needed per homogenous soil parcel,
which is in the order of one ha. If one is to avoid deploying extra nodes for
the sole purpose of relaying traffic, a radio with communication range above
the average performance of wireless sensors is to be used. We finally opted for
the tinynode \cite{tinynode} platform, which allowed us to obtain a
communication range of 200m and above in a consistent manner.

\textbf{Cluster-based Hybrid Architecture:} The interconnection of far-apart
clusters with the centralized server necessitated the design of a hybrid
architecture with the cluster heads implementing a bridge to the server. In the
absence of cellular phone coverage, we implemented in a first phase a IEEE
802.11 bridge. As GSM coverage improved in 2007, we migrated to a GPRS-based
bridge that removes the necessity to maintain a local server at the deployment
site.

\textbf{Web-based Interface for Data Retrieval:} We developed a web-based
application for the retrieval of cluster-based information (such as maps and
per node information) as well as individual sensors data display and download.
This application can be accessed at: http://csn.epfl.ch.


==> discussion.tex <==
\section{Discussion}
Potential users expressed keen interest in several cases. In particular, a
major NGO working in the field of dry-land farming throughout India expressed
interest in the WSN technology. Such promising results must be tempered by the
low response obtained by the application use, which we address in section
\ref{usage}.
\subsection{Usefulness}
From the questionnaires, there is a large consensus as to the utility of using
finer-grained environmental data for rain-fed agriculture.

The level of detail, at which scientists answered the on-line survey indicates
a high level of interest and curiosity on their part. Such an interest was
already perceptible at the inception of the project. However, the creation of
precise use case was not possible then.

This gap was filled during the individual interviews with scientists coming
from academia, as well as the non-governmental sector. With four precise use
cases and potential partners clearly identified, the initiative is now in the
hands of the information and communication systems specialists.

One central question is the potential of information-sharing with farmers. Will
the results ever leave the lab and scientific reports to materialize in the
field? According to our interviews with government officials
\cite{PanchardRS08}, the Indian institutional framework is very clear: The
agriculture scientists are expected to provide scientific evidence of
phenomena, to investigate preventive or corrective actions when appropriate,
and to publish recommendations that are used by the agriculture department to
relay information to the public (which is referred to as extension work). The
case of the non-governmental sector is different. Large NGOs are conducting
applied research aimed at improving farming practices in dry-land management.
In this case, the scientists work directly in contact with the farmer. This
makes them privileged partners.

\subsection{Usability}
New types of sensors were mentioned in the course of the experiment. Most
prominently, in-situ chemical sensors that could sense the concentration of
nutrients (nitrogen, phosphorus, potassium) in the soil are mentioned
repeatedly. The development of such sensors is still at an experimental stage,
but some recent advances have been made for low-cost sensors using
ion-selective electrodes \cite{KimHSM07}.
%
%Bio-sensors are also the object of the interest of microbiologists and
%entomologists.

The accuracy is a recurring concern. However, the exact precision to which
sensors need to operate is still an open question. In general, it is more
important to be roughly right than precisely wrong.

Parameters linked with the soil are pinpointed as having a high space
variability. As a consequence, any high-precision technology that comes at a
price such that it is not possible to diversify the readings is not going to be
usable. With low cost sensors, a relatively high error can be compensated by
spatial diversity, which allows for the statistical elimination of outlying
measurements.
%This is acknowledged by the respondents, who ask for a distinctively higher
%spatial resolution for soil moisture than for other parameters.

The sampling period of the data (time variability) is still the object of
uncertainty. Measures shorter than a day are not a priori taken into
consideration by scientists in the framework of an applied research for
agriculture. At present, the researchers mostly want daily data, since they use
data of similar granularity  obtained from conventional measurements without
sensors. During debriefing sessions, however, we gathered evidence that the
responses are likely to change with time spent on reflection and experience
with high-resolution  data. Indeed, when prompted by one of the authors with
background in agriculture about possible uses for research, the participants
acknowledge in a majority of cases that such data could be used in the
framework of their research.

It appears that certain elements of  the current responses, particularly those
related to time resolution, will change after some experience and / or
contemplation on use of high time resolution data. Researchers have always
viewed data gathering as a major constraint in research design and
conceptualization. The current experiment presents a completely contrasting
situation with the provision of very rich data in both time and space for
parameters of interest. It is in this light that we suggest a co-learning
process for agriculture researchers and sensor technology providers to evolve
better and meaningful use cases.
%
%On the technical side, more work has to be done to integrate new, more complex
%sensors to the current data acquisition kit.

\subsection{Use} \label{usage}
We tried to provide possible explanations about the paradoxical low level of
use recorded during the experiment. It cannot be ruled out that this reflects
the actual disinterest of the participants. However, that would be
contradictory with all the other results of the survey.

Moderate computer literacy is a possible explanation. A similar result was
obtained during a previous experiment conducted in 2006, specifically about
interface design \cite{Panchard06}. At that time, we had seen a clear
difference of behavior between scientists used to working with environmental
sensors and computers, and those who did not have this expertise. As a
consequence, we sought to improve the interface, but such a gap remains, as
illustrated by the difference in handling the application from senior
scientists and their younger, computer-savvy students.

However, this is only a partial explanation to the observed phenomenon. As a
matter of fact, despite their computer literacy the students and post-docs did
not extensively use the application. A posteriori, this can be explained by the
difficulty in finding a one-size-fits-all scenario for the participants of the
survey. We had not realized how diverse the concerns of agricultural scientists
could be. It is likely that the questions asked made little sense to most of
the participants to the survey.

%\subsection{Sectoral analysis}
%It is interesting to analyze the response of the participants based ont heir
%background. Most prominently, the position of the joint-director of the
%agriculture department of Karnataka state was clear. Conducting applied
%research is beyond the mandate of a governmental agency, which is only
%concerned by extension, i.e. information relaying from the scientific community
%to the farmers.
%
%This categorical response illustrates the functioning of the Indian public
%sector when it comes to design and implementation of policies
%(\textbf{cross-checking necessary here}). The academic institutions are
%expected to provide scientific evidence of phenomena, to investigate preventive
%or corrective actions when appropriate, and to publish recommendations. The
%administrative role is one of information spreading and relaying to the public
%(which is referred to as extension work), and of control. A valid concern to
%raise at this point is to question how the information is collected and
%forwarded in the other direction, in our case, how do the needs and wishes of
%the farmers come to the scientific's desk. But we did not investigate this
%question.
%
%The case of the non-governmental sector is different. Large NGOs do not
%restrict themselves to extension and implementation. As we found out, BAIF, for
%instance, is conducting applied research aimed at improving farming practices
%in dry-land management. In this case, the scientist works directly in contact
%with the farmer. This makes him or her a privileged partner in the field.
%
%We did not extend our survey to the industry of agriculture inputs or to
%corporate agriculture, although these two sectors are likely users of the
%wireless sensor networking technology. In the first case, we did not want to
%get involved in the controversy surrounding the effects of large seeds
%providers on the livelihood of small and marginal farmers in India. In the
%second case, the type of agriculture practiced (mechanized farming, on-demand
%irrigation, precision agriculture with high added-value) was considered too
%different from our focus of interest, namely rain-fed farming.


==> introduction.tex <==
\section{Introduction}
Today emerging countries face the antagonistic goals of developing their
economies and improving their population's livelihood, while sustaining their
natural resources and environment. Environmental monitoring seems to hold great
promise for tackling these issues. One typical example is air pollution
monitoring, because this is a major concern in many urban areas of developing
countries, especially in the mega cities of Asia. Water quality control is
another opportunity: in developing countries, diarrhoeal diseases consecutive
to the consumption of contaminated water are one of the main causes of child
mortality.

Most of all, agriculture comes as a natural application, given the importance
that climatic and physical parameters have throughout the development of the
crop. Indeed, developing countries often have to cope with a large farming
population who have seen their situation deteriorate in recent years due to the
instability of market prices and the perceived effects of climate change.

As a typical example, the share of agriculture for employment in India is about
67\%, with a majority of small land holdings. In Karnataka (Southern India),
87\% of the farms have less than 4 ha and account for more than 50\% of the
total cultivated land, while 39\% of the total are very small farms (less than
1 ha). These \emph{resource-poor} farmers usually lack access to irrigation
facilities and depend on rain-fed farming for their livelihood
\cite{DiwikaraC07}. Their crop yields are highly \emph{unreliable}, due to the
variability in both the total rainfall and its distribution \cite{GadgilAR99,
Abrol96}. Unlike industrial farming companies, they face daunting challenges,
as is illustrated by the current wave of suicides throughout the country
\cite{Mishra06}.

We performed a survey in 2004 to identify the user needs of the rural
population in three small villages of Karnataka \cite{RaoGRG04}: the themes of
crop yield prediction, pest and disease control, and water levels in bore wells
stood out prominently among farmers' responses. Practicing exclusively rain-fed
farming, they would greatly benefit from a better knowledge of the field
environment, and from more adapted strategies and practices.

To address these issues, it seems natural to assess the potential of wireless
sensor networks (WSNs), in particular, the increased space and time resolution
they bring to environmental data at an affordable price. WSNs are today viewed
as an enabling technology for precision agriculture: irrigation management,
frost prevention, nutrient or pesticides control are documented examples
\cite{WarkCSKGCVSB07}. Still, it remained to be proven whether a similar
knowledge could be used by the population who needs it most: the resource-poor
farmers who practice rain-fed agriculture.

This has been the endeavor of the COMMON-Sense Net \cite{PanchardRPHJ07}
project, which has investigated over three years the utilization of WSNs as a
decision-support tool for rain-fed farming. Our goal was to help the farmers
monitoring the physical farming environment, in order to understand more
precisely the physical processes at hand, and to react optimally to changing
conditions.

Our vision has been to bring the benefits of technology \emph{directly} to
farmers, in a participatory way. We deployed our system, described in
Sec.~\ref{sectioncsn}, after identifying use cases with the locals. Over a long
period of data collection and usage, we reached an impasse: numerous
difficulties have emerged, essentially hindering our efforts to bring in a
participatory manner the added value of WSN technology, through our system, to
the farmers.

This has been primarily due to the farmers' alienation with the worlds of
science and technology. Presenting the lessons learned through our three-year
long effort and deployment, in Sec.~\ref{sectionlessons}, we are currently
forced to consider as somewhat idealistic our initial objective. The
resource-poor farmers could not really put enhanced environmental data in use
effectively.

Based on these experiences, we moved on with a different approach: we
investigate controlled-environment strategies related to rain-fed farming, such
as developing new crop varieties or pest prediction measures. Accordingly, the
\emph{position} this paper takes is as follows: \emph{Under the current
conditions in developing regions, such as Karnataka, the targeted users for
WSN-enabled applications, should be researchers, scientists, and technicians}.
As our study case, long experience, and recent experiment we conducted in
Bangalore, from November 2007 to February 2008, indicate, this orientation
towards a new user group (of scientists) that can then advise or guide the
farmers appears currently the only method to have an effective decision-support
system for rain-fed farming.

This article brings this seemingly pessimistic yet realistic position to the
attention of the community. Essentially, our concerted effort of deploying and
running the COMMON-Sense Net system points that still scientists remain the
preferred 'customers' of WSN technology. We present the learned lessons that
led us to this shift away from our initial objective. Then,
Sec.~\ref{sectionexperiment} describes the methodology for our user experiment
to determine if our new user target group was an appropriate choice. In
Sec.~\ref{sectionresults}, we present our results, followed by a discussion,
future work and conclusions.


==> jam.tex <==
%**************************************************************
\chapter{A Wireless Sensor Network Toolkit for Rural India} \label{chap:csn_deployment}
%**************************************************************
(...)

\section{Human issues}
In order to achieve the successful implementation of the uses cases described
in chapter~\ref{chap:user_needs}, the collaboration of the farmers was required
to protect the hardware, to report regularly on field conditions and to give
feedback on the added value brought by the technology. Unfortunately, we
observed an initial distrust of the population towards the technology and the
presence of scientists in the field.

Informal discussions with local stake-holders indicated that the population of
small farmers has an experience of being systematically left behind in the
innovation process. A second obstacle was the difficulty to translate the
scientific terminology of environmental science (soil moisture,
evapotranspiration, etc.) into the language of the field. Finally, the current
uncertainty about the benefit to cost ratio of the technology did not encourage
active collaboration.

In 2007, CEDT reassessed the situation in an internal project
document\cite{Jamadagni07}. Informal interviews with some marginal farmers
indicated that they are not interested in any project that does not bring them
rains, road to village, a perennial bore well, or cash (as loans for example)
and subsidies.

In this assessment, the results of the survey on information
needs\cite{RaoGRG04} were not deemed invalid, but considered in the light of
the circumstances:

\begin{enumerate}
  \item Farmers were asked to think about a very specific question, which might
bear limited relevance in the face of more immediate problems, in particular
the threat of bankruptcy.
  \item There if a minority of individuals who recognize the commitment of scientists
to improve farming conditions through this project. However, their importance
was exaggerated in the survey because they were the ones more willing to
participate actively to the survey
  \item Farmers tend to have confidence in Mr. Sheshagiri Rao (our ``hybrid''), because he is one of them
\end{enumerate}

In three occasions, we experienced theft of hardware. Although such events
could not be traced with certainty to the local population, the Chennakeshava
Trust eventually concluded to the necessity of locking the hardware in
protected chambers in order to prevent more stealing. This clearly contradicts
the initial goal of using a participatory approach, and also conflicts with the
flexibility required of a light-weight system.


==> lessonslearned.tex <==
\section{Lessons Learned} \label{sectionlessons}
Deploying a sparse network in a remote and uncontrolled environment raised
critical deployment issues. Fluctuations of the radio channel caused by the
growth of vegetation during the cropping season had a severe impact on the
network connectivity. To diagnose such problems and other software or hardware
failures would require a constant presence of communication engineers on the
deployment site, which is difficult to achieve in a rural setting.

%\begin{itemize}
%  \item fluctuations of connectivity due to the limited number of neighbors,
%  \item fluctuations of connectivity due to the evolution of the
%  environment, especially the growth of the vegetation during the cropping
%  season,
%  \item hardware and software failures that are difficult to trace,
%  \item unreliability of the power grid, which affects the performance of the local
%  server and WiFi access point (rural India is characterized by frequent and long power
%  cuts).
%\end{itemize}

The main lesson to be learned from this deployment, however, was the difficulty
of implementing and testing convincingly our use cases in the field. In order
to achieve this, the collaboration of the farmers was required to protect the
hardware, to report regularly on field conditions and to give feedback on the
added value brought by the technology. Unfortunately, we observed an initial
distrust of the population towards the technology and the presence of
scientists in the field.

Informal discussions with local stakeholders indicated that the population of
small farmers has an experience of being systematically left behind in the
innovation process. A second obstacle was the difficulty to translate the
scientific terminology of environmental science (soil moisture,
evapotranspiration, etc.) into the language of the field. Finally, the current
uncertainty about the benefit to cost ratio of the technology did not encourage
active collaboration.

%As a consequence, we reached the following deadlock, specifically the necessity
%to produce compelling use cases to convince the farmers, and at the same time
%the necessity to rely on the farmers in order to develop the same use cases.

Both the difficulty to trace the technical problems and the impossibility to
create a partnership with farmers represented serious obstacles. This called
for a change of paradigm: in our experience, the promise of ubiquitous
computing will have to wait for maturation of both the technology and the users
before being fulfilled. Instead, managing the technology in a controlled
environment with the participation of committed users can lead to rapid
results, provided we can ensure a spill-over effect on the farming population.
In the next section, we explain why we decided to focus on scientists working
on applied research for rain-fed agriculture, and how we verified the
appropriateness of this new approach.


==> relatedwork.tex <==
\section{Related work}
What to put here?

